Euphonic: inelastic neutron scattering simulations from force constants and visualisation tools for phonon properties

Interpretation of vibrational inelastic neutron scattering spectra of complex systems is frequently reliant on accompanying simulations from theoretical models. Ab-initio codes can routinely generate force constants, but additional steps are required for direct comparison to experimental spectra. On modern spectrometers this is a computationally expensive task due to the large data volumes collected. In addition, workflows are frequently cumbersome as the simulation software and experimental data analysis software often do not easily interface to each other. Here a new package, Euphonic, is presented. Euphonic is a robust, easy to use and computationally efficient tool designed to be integrated into experimental software and able to interface directly with the force constant matrix output of ab-initio codes.

==> latexmkrc <==
# Allows referencing labels across different files (e.g. main.tex and supplementary.tex)
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
